Introducing explainable supervised machine learning into interactive feedback loops for statistical production system

Statistical production systems cover multiple steps from the collection, aggregation, and integration of data to tasks like data quality assurance and dissemination. While the context of data quality assurance is one of the most promising fields for applying machine learning, the lack of curated and labeled training data is often a limiting factor. The statistical production system for the Centralised Securities Database features an interactive feedback loop between data collected by the European Central Bank and data quality assurance performed by data quality managers at National Central Banks. The quality assurance feedback loop is based on a set of rule-based checks for raising exceptions, upon which the user either confirms the data or corrects an actual error. In this paper we use the information received from this feedback loop to optimize the exceptions presented to the National Central Banks thereby improving the quality of exceptions generated and the time consumed on the system by the users authenticating those exceptions. For this approach we make use of explainable supervised machine learning to (a) identify the types of exceptions and (b) to prioritize which exceptions are more likely to require an intervention or correction by the NCBs. Furthermore, we provide an explainable AI taxonomy aiming to identify the different explainable AI needs that arose during the project.

==> CSDBML/myscellaneous.tex <==

\subsubsection{Building Trust}
Despite the careful testing and calibration of the machine learning process by the \emph{data scientists}, \emph{end users} of the data can identify potential data issues that have not been raised by the algorithm. These issues are communicated via the Data Quality Managers (DQM) to the statistical production team (comprising of \emph{business experts} and \emph{data scientists}) responsible for the CSDB data quality \cite{csdb_ml}.

The first step for the statistical production team is to verify that indeed the issues identified are not flagged by the algorithm. The next step is to investigate the reasoning behind this choice from the perspective of the algorithm by determining: $(i)$ similar instances in the training dataset \cite{case_based_explanation}, $(ii)$ which features contributed to the decision \cite{shapTree,ribeiro2016why} (cf. Figure~\ref{fig:fig}) and $(iii)$ local decision rules to better understand the model logic \cite{lore,Ribeiro2018AnchorsHM}.



\begin{figure}[tb]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=.8\linewidth]{images/Shap_waterfall.png}
  \caption{Local feature importance for a given instance\cite{shapley}}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=.8\linewidth]{images/Shap_mean.png}
  \caption{Global Feature Relevance}
  \label{fig:sub-second}
\end{subfigure}
\caption{Shapley feature values by TreeExplainer \cite{shapTree}}
\label{fig:fig}
\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=.8\linewidth]{images/lime.png}
%    \caption{Local approximation for feature importance by Lime \cite{ribeiro2016why}}
%    \label{fig:my_label}
%\end{figure}
\subsubsection{Actionable Insights}

Following the formulation from Utsun et~al.~\cite{utsun_linear_recourse} and  the available open source implementation \cite{dice}, we quantified the relative difficulty in changing a feature through the application of weights to the  counterfactual explanations algorithm. For instance, in our case,  recommendations should not ask the \emph{business expert} (DQM) to modify the country in which a financial instrument was issued or change the issue date to a time before the creation of the issuing company (cf. Figure~\ref{fig:counterfactual}).

\begin{figure}[bt]
    \centering
    \includegraphics[width=.6\linewidth]{images/counterfactual.png}
    \caption{Set of counterfactual decisions generated \cite{lore,dice}}
    \label{fig:counterfactual}
\end{figure}




%\subsubsection{Gain Knowledge}
%During our work, after several models and feature attribution visualizations, we noted that what was happening with our data was not what we expected but users were doing other things.

\subsubsection{Model Monitoring}
Detecting when the underlying distribution of the data changes is paramount for this use case, since failing to predict outliers or errors in the data will lead to a drop in the trust of the machine learning model. Also, the risk of having an incoherent explanation through time caused by the continual learning process is utterly important, a discrepancy will lead to a decrease of trust by the \emph{business experts}. 

An approach suggested by Lundberg et~al.~\cite{shapTree} is to monitor the SHAP value contribution of input features over time together with decomposing the loss function across input features in order to identify possible bugs in the pipeline.


\begin{figure}[tb]
    \centering
    \includegraphics[width=.6\linewidth]{images/monitoring.png}
    \caption{Simulated covariate distribution shift detected by local attribution of Shapley values in one of the descriptive features }
    \label{fig:local_monitoring}
\end{figure}

In Figure~\ref{fig:local_monitoring}, we can see the local contribution of SHAP values through time for a continuous feature. The drop of Shapley contributions denotes a possible distribution change for a given feature or a change in the model's inner working that needs human assistance for further evaluation of performance and explainability ~\cite{shapTree}. 

\subsubsection{Fostering Explanations through Simple Models}
Following the notation of paragraph \ref{sec:simple_models}, for our case the original model $f_O(X)$ is a catboost classifier~\cite{dorogush2018catboost,prokhorenkova2019catboost} which is a gradient boosting model~\cite{gbm} that often achieves state of the art results in many different types of problems \cite{supervised_learning_algorithms,gbm_travel} and the copied models $f_C(X)$ are a scikit-learn~\cite{scikit-learn} decision tree classifier and a Generalized Linear Model (GLM). The simpler models are of slightly inferior quality  (cf. Table~\ref{tab:table-name}). However, having two simple models helps to improve the overall global explainability for the \emph{data scientist} and to simplify deployment.


\begin{table}[bt]
\centering
\caption{Catboost is the original model $f_O(X)$ and the Decision Tree and the Generalized Linear Model the  copied classifier $f_C(X)$}
\label{tab:table-name} 
\begin{tabular}{lccc}
\toprule
          & Catboost & Decision Tree & GLM \\ %\hline
\midrule
AUC       & 0.816    & 0.771         & 0.741        \\
Precision & 0.805    & 0.741         & 0.685        \\
Recall    & 0.833    & 0.824         & 0.733   
\\
\bottomrule
\end{tabular}
\end{table}


%Providing statistical data and information of the highest quality is a core task at the European System of Central Banking (ESCB).  Assuring the quality of data in  statistical production systems is crucial  as it becomes the input to many later decisions, that is why it has relied on domain  experts with profound understanding of the data. These experts ensure that the information used in the compilation of statistical products is of the highest quality based on their expertise in the specific fields.
%Through their experience of their respective financial or otherwise market they have made sure that the information used in the compilation of the statistical products is of high quality.

%The benefit of using expert knowledge for quality assurance of statistical products is  two-fold: $(i)$ all the knowledge and expertise of the domain experts is reflected in the final data and $(ii)$ the overall confidence about the final product increases on the side of the producers and consumers of official statistical data. However,  as the volume and granularity of the data increases, this process becomes more and more difficult to maintain (\textit{scaling up}). It is almost impossible to manually assess the quality of granular data  without substantially increasing the number of experts.

%Over the years various approaches have been developed to support and automate the quality assurance procedures. However, these approaches have limitations themselves:
%\begin{itemize}
%    \item \textbf{Data aggregation:} Assessing the quality of the data based on an aggregated level, condenses the information that needs to be checked to a manageable amount. The disadvantage of this approach is that aggregation might hide granular data quality issues on the level of individual observations. The risk of obfuscation depends on the type and level of aggregation used.
%    \item \textbf{Static quality rules:} Another way to ensure data quality for a big data scenario, is using a fixed set of rules to identify potential quality issues. These rules are based on expert knowledge and formalise certain aspects of their domain knowledge. This method flags micro data that, for instance, surpass a pre-defined  threshold. The flagged observations typically represent only a small fraction of the entire data set, allowing the field experts to focus their analysis on a limit amount of data. The shortcoming of this approach is that relying on a fixed set of static rules is not flexible enough to capture dynamics in data nor does it automatically adjust to new insights provided by users. 

%\end{itemize}


%Both of the aforementioned approaches can be useful, but they have clear limitations. Aggregation can hide granular data quality issues which could become visible if a different type of aggregation is selected by the data users, while relying on fixed set of rules is not flexible enough to capture changes in the data nor does it adjust to new user input. 

In order to maintain high standards of quality assurance, it is crucial to identify new approaches that address these limitations. In this paper we present an approach to utilize machine learning with the goal of establishing dynamic rules that take into account user feedback. We leverage the feedback from data quality reviews to establish a feedback loop which can serve as input to the machine learning solutions. This feedback loop helps to capture and formalise expert knowledge. Our use case is the Centralised Securities Database (CSDB) which already incorporate an integrate data quality tool and thereby provides the necessary infrastructure for establishing a feedback loop.

Utilizing the historical actions performed by the experts, we build and evaluated a machine learning model to optimize the discovery and resolution of potential quality issues. Such a model can support the work of the data compilers and quality managers at  National Central Banks.


\subsection{Building Trust}
Despite the careful testing and calibration of the machine learning process by the \emph{data scientists}, \emph{end users} of the data can identify potential data issues that have not been raised by the algorithm. These issues are communicated via the Data Quality Managers (DQM) to the statistical production team (comprising of \emph{business experts} and \emph{data scientists}) responsible for the CSDB data quality \cite{csdb_ml}.

The first step for the statistical production team is to verify that indeed the issues identified are not flagged by the algorithm. The next step is to investigate the reasoning behind this choice from the perspective of the algorithm by determining: $(i)$ similar instances in the training dataset \cite{case_based_explanation}, $(ii)$ which features contributed to the decision \cite{shapTree,ribeiro2016why} (cf. Figure~\ref{fig:fig}) and $(iii)$ local decision rules to better understand the model logic \cite{lore,Ribeiro2018AnchorsHM}.



\begin{figure}[tb]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=.8\linewidth]{images/Shap_waterfall.png}
  \caption{Local feature importance for a given instance\cite{shapley}}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=.8\linewidth]{images/Shap_mean.png}
  \caption{Global Feature Relevance}
  \label{fig:sub-second}
\end{subfigure}
\caption{Shapley feature values by TreeExplainer \cite{shapTree}}
\label{fig:fig}
\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=.8\linewidth]{images/lime.png}
%    \caption{Local approximation for feature importance by Lime \cite{ribeiro2016why}}
%    \label{fig:my_label}
%\end{figure}
\subsection{Actionable Insights}


Following the formulation from Utsun et~al.~\cite{utsun_linear_recourse} and  the available open source implementation \cite{dice}, we quantified the relative difficulty in changing a feature through the application of weights to the  counterfactual explanations algorithm. For instance, in our case,  recommendations should not ask the \emph{business expert} (DQM) to modify the country in which a financial instrument was issued or change the issue date to a time before the creation of the issuing company (cf. Figure~\ref{fig:counterfactual}).

\begin{figure}[bt]
    \centering
    \includegraphics[width=.6\linewidth]{images/counterfactual.png}
    \caption{Set of counterfactual decisions generated \cite{lore,dice}}
    \label{fig:counterfactual}
\end{figure}




%\subsubsection{Gain Knowledge}
%During our work, after several models and feature attribution visualizations, we noted that what was happening with our data was not what we expected but users were doing other things.

\subsection{Model Monitoring}
Detecting when the underlying distribution of the data changes is paramount for this use case, since failing to predict outliers or errors in the data will lead to a drop in the trust of the machine learning model. Also, the risk of having an incoherent explanation through time caused by the continual learning process is utterly important, a discrepancy will lead to a decrease of trust by the \emph{business experts}. 

An approach suggested by Lundberg et~al.~\cite{shapTree} is to monitor the SHAP value contribution of input features over time together with decomposing the loss function across input features in order to identify possible bugs in the pipeline.


\begin{figure}[tb]
    \centering
    \includegraphics[width=.6\linewidth]{images/monitoring.png}
    \caption{Simulated covariate distribution shift detected by local attribution of Shapley values in one of the descriptive features }
    \label{fig:local_monitoring}
\end{figure}

In Figure~\ref{fig:local_monitoring}, we can see the local contribution of SHAP values through time for a continuous feature. The drop of Shapley contributions denotes a possible distribution change for a given feature or a change in the model's inner working that needs human assistance for further evaluation of performance and explainability ~\cite{shapTree}. 

\subsection{Fostering Explanations through Simple Models}
Following the notation of paragraph \ref{sec:simple_models}, for our case the original model $f_O(X)$ is a catboost classifier~\cite{dorogush2018catboost,prokhorenkova2019catboost} which is a gradient boosting model~\cite{gbm} that often achieves state of the art results in many different types of problems \cite{supervised_learning_algorithms,gbm_travel} and the copied models $f_C(X)$ are a scikit-learn~\cite{scikit-learn} decision tree classifier and a Generalized Linear Model (GLM). The simpler models are of slightly inferior quality  (cf. Table~\ref{tab:table-name}). However, having two simple models helps to improve the overall global explainability for the \emph{data scientist} and to simplify deployment.


\begin{table}[bt]
\centering
\caption{Catboost is the original model $f_O(X)$ and the Decision Tree and the Generalized Linear Model the  copied classifier $f_C(X)$}
\label{tab:table-name} 
\begin{tabular}{lccc}
\toprule
          & Catboost & Decision Tree & GLM \\ %\hline
\midrule
AUC       & 0.816    & 0.771         & 0.741        \\
Precision & 0.805    & 0.741         & 0.685        \\
Recall    & 0.833    & 0.824         & 0.733   
\\
\bottomrule
\end{tabular}
\end{table}



\subsection{Meta-Classifier}

In our experiments we concluded that having a machine learning model per exception type is the
recommended strategy for this project. Because the training data for the models primarily comes from a different origin than
the gold dataset (bulk tool audits vs. exceptions from iDQM rules), the accuracy of the trained models is reduced. To improve the precision of the models, a threshold for the probabilities can be applied, such as
only samples which are classified with high certainty get the label “anomalous”. For the gain in the precision
it must be taken into account that the recall is decreasing.
An evaluated solution was to pipe the prediction of the several models, the probability of containing a
specific exception, to a second machine learning model. This second model is the meta-classifier, which was
in our case a multiclass Logistic Regression (see also section 4.2). It predicts for a record the probability for
containing a specific exception type or to be nominal. The Logistic Regression acts like a tool that
automatically determines the right threshold of the provided anomaly-probability for the gold dataset. It
has also the side-effect, that the probabilities of the models may help to improve the accuracy of each
other. In this sense, the logistic regression as a meta-classifier acts as an automatic calibration of the
individual model probabilities.

An improved solution would use a multinomial Logistic Regression to satisfy the property that an
instrument fact record can contain more than one data issue. This approach was not evaluated as it would
need extra effort to prepare data for having the proper labels.
Especially in earlier versions of the models, which were trained with low quality data, this meta-classifier
improved the precision significantly. In the current solution, the difference is not so astonishing but it still
brings a little improvement for some exception types. The improvement is often comparable with ranking
the samples by probability and evaluating on the first k samples, which acts like an implicit setting of the
threshold for the probability.

\begin{figure}[ht]
    \centering
    \includegraphics[width=.8\linewidth]{images/metaclass.png}
    \caption{ Abstract scheme showing how the Meta-Classifier is integrated with the binary models}
    \label{fig:my_label}
\end{figure}




==> CSDBML/relatedWork.tex <==
\section{Related Work}

(tbd, suggested structure)

\begin{itemize}
    \item DQA processes in official statistics - (GEORGIOS)
    \item Use cases of ML for DQA in official statistics
    \item XAI taxonomy or requirement engineering
    \item (maybe) methods relevant for the task at hand (L2R, Catboost, etc.)
\end{itemize}

The state of the art of ML applications have to two requirements: high performance and model explainability.

Explainable AI methods are encountering what appears to be ill-defined evaluation methods \cite{rigorousXAI}, yet Machine learning conferences publish papers that wield the term in a quasi-mathematical way \cite{mythos_interpretability}. Some authors state that there might be a gap between scientific research in explainable ML and real-world use cases \cite{explainable_public_policy,bewareInmates}. There are few real explainable machine learning use cases, previous work found on the literature  relies either on theoretical problems or toy problems \cite{ATI_taxonomy}.
To the best of our knowledge there is no previous work done on explainable machine learning cases for data quality assurance applications in the public policy sector. 

The novelty of our paper regarding explainable AI relies on introducing a well-defined set of explanation needs on a real world use case and providing one use case more for explainable AI: interaction feedback loops in statistical production systems.
